Regulating Autonomous Mobility-on-Demand Operators with Fixed and Adaptive Penalties: A Multi-Agent Reinforcement Learning Approach

Profit-maximizing Autonomous Mobility-on-Demand (AMoD) operators may exploit consumer surplus through excessive prices and underserve less profitable regions by relocating vehicles away from them. We study how penalty-based regulation of an AMoD operator in a multimodal mobility system can limit surge pricing and improve regional service availability. We model regulation as an outer control loop that acts on a learning-based operator. Static regulation with fixed penalties is formulated as a Markov Decision Process for an operator that jointly controls pricing and rebalancing, and dynamic regulation as a Partially Observable Stochastic Game in which a regulator periodically adjusts region-specific penalties in closed loop. Operator and regulator policies are learned with graph-based multi-agent reinforcement learning. In experiments with real-world Manhattan data, fixed surge pricing penalties reduce the share of travelers facing excessive prices from 22% to 1%. For regional service availability, dynamic regulation improves the regulator's reward by up to 15.6% over fixed penalties of equal mean intensity. The gains in service availability are strongest when spare fleet capacity exists, whereas service deficits persist in peak periods with highly utilized fleets. The learned regulator policy responds by reducing penalties where limited fleet capacity restricts compliance. The results identify trade-offs between regulatory targets, operator profitability, and traveler utility.

==> abbreviations.tex <==
\newacronym{acr:amod}{AMoD}{autonomous Mobility-on-Demand}
\newacronym{acr:mod}{MoD}{Mobility-on-Demand}
\newacronym{acr:pt}{PT}{public transport}
\newacronym{acr:msp}{MSP}{mobility service provider}
\newacronym[longplural={municipal transportation authorities}]{acr:mta}{MTA}{municipal transportation authority}

\newacronym{acr:mpc}{MPC}{Model Predictive Control}
\newacronym{acr:ppo}{PPO}{Proximal Policy Optimization}

\newacronym{acr:mdp}{MDP}{Markov Decision Process}
\newacronym{acr:posg}{POSG}{Partially Observable Stochastic Game}

\newacronym{acr:drl}{DRL}{deep reinforcement learning}
\newacronym{acr:rl}{RL}{reinforcement learning}

\newacronym{acr:sac}{SAC}{Soft Actor-Critic}
\newacronym{acr:a2c}{A2C}{Advantage Actor-Critic}
\newacronym{acr:td}{TD}{temporal-difference}

\newacronym{acr:gcn}{GCN}{graph convolutional network}
\newacronym{acr:fc}{FC}{fully connected}
\newacronym{acr:lrelu}{LeakyReLU}{Leaky Rectified Linear Unit}
\newacronym{acr:relu}{ReLU}{Rectified Linear Unit}

\newacronym{acr:fcfs}{FCFS}{first-come, first-served}
\newacronym{acr:od}{OD}{origin-destination}

\newacronym{acr:gtfs}{GTFS}{General Transit Feed Specification}
